Using an Automated Heterogeneous Robotic System for Radiation Surveys

During missions involving radiation exposure, unmanned robotic platforms may embody a valuable tool, especially thanks to their capability of replacing human operators in certain tasks to eliminate the health risks associated with such an environment. Moreover, rapid development of the technology allows us to increase the automation rate, making the human operator generally less important within the entire process. This article presents a multi-robotic system designed for highly automated radiation mapping and source localization. Our approach includes a three-phase procedure comprising sequential deployment of two diverse platforms, namely, an unmanned aircraft system (UAS) and an unmanned ground vehicle (UGV), to perform aerial photogrammetry, aerial radiation mapping, and terrestrial radiation mapping. The central idea is to produce a sparse dose rate map of the entire study site via the UAS and, subsequently, to perform detailed UGV-based mapping in limited radiation-contaminated regions. To accomplish these tasks, we designed numerous methods and data processing algorithms to facilitate, for example, digital elevation model (DEM)-based terrain following for the UAS, automatic selection of the regions of interest, obstacle map-based UGV trajectory planning, and source localization. The overall usability of the multi-robotic system was demonstrated by means of a one-day, authentic experiment, namely, a fictitious car accident including the loss of several radiation sources. The ability of the system to localize radiation hotspots and individual sources has been verified.

==> text/methods-radiation-ugv.tex <==
\subsection{Terrestrial Radiation Mapping}

\hl{TomL // Mereni radiace z UGV} 


==> text/results-experiment.tex <==
\subsection{Result Summary}

\hl{Vsichni // Souhrnne vysledky, jak se povedl experiment jako celek, casova osa jednotlivych fazi (Gantt graph)} Figure \ref{fig:gantt}; \hl{souhrny prehled mapovych vrstev} Figure \ref{fig:map-layers}

Entire experiment, as presented within this article, was carried out during 24 hours. This continuous time interval included not only the necessary objectives, namely the data gathering and processing, but also site preparation and cleanup, safety concerns, and tasks not related with the experiment. The time-demands of the operations relevant to the robotic radiation mapping and source localization are summarized in the Gantt chart in Figure~\ref{fig:gantt}. It is clearly visible that \hl{co trva nejdyl? jsou v tom zahrnuty i vstupy uzivatele a manipulace?}

\begin{figure*}[!tbp]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/gantt.PNG}
	\caption{The approximate duration of the individual tasks conducted during the experiment. \hl{Probrat podobu, kazdy musi dodat doby trvani svych casti.}}
	\label{fig:gantt}
\end{figure*}



\begin{figure}[!tbp]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/map-layers2.png}
	\caption{The major map layers assembled during the mapping and processing. The layers are time-ordered from the bottom: the primary orthophoto (a); UAS-based, shaded DEM (b); UAS-based orthophoto (c); UAS-based radiation map (d); detected regions of interest (e); DEM-based UGV traversability map (f); UGV-based radiation map (g). [1-column figure]}
	\label{fig:map-layers}
\end{figure}


==> text/results-trajectory-uas.tex <==
\subsection{UAS Trajectory}

According to the algorithm described in section~\ref{ssec:aerial-rad-map}, we automatically adjusted the vertical components of the trajectory for the aerial radiation mapping utilizing the DEM obtained within previous step. At first, the trajectory (Figure~\ref{fig:uas-traj-rad-plan}) was split into the 10~m segments resulting in 209 waypoints; subsequently MSL height for every waypoint was computed (red points in Figure~\ref{fig:rad-traj-profile}).

\begin{figure*}[!tbp]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/rad-traj-profiles.png}
	\caption{The vertical profile of the UAS trajectory during the radiation-mapping phase together with the trajectory waypoints and underlying terrain (upper part). AGL flight height measured by rangefinger, and its GPS/DEM based estimation is shown in the bottom part.}
	\label{fig:rad-traj-profile}
\end{figure*}

Compared with the photogrammetry flight, the second UAS flight lasted longer, 20~minutes approximately, due to the trajectory length and lower operation speed. Thanks to the GPS receiver and laser rangefinder, components integrated in onboard radiation detection system, we can analyse the 'terrain following' algorithm performance. Upper part of the Figure~\ref{fig:rad-traj-profile} displays the vertical coordinate of the actual GPS trajectory and underlying terrain; the bottom part depicts height above ground level. The presented data show us the UAS flown in relatively constant distance from the surface, however, in some moments, deviation from the desired value of 15~m is obvious. Rangefinder reports the height of 13.7~m RMSE, the GPS derived value is, on the other hand, slightly higher -- 16.6~m RMSE. It should be noted that both data sources are not accurate enough for detailed assessment: the rangefinder measures wrong distance during UAS tilting, and both GPS and DEM error lies in meter order. Despite that facts, the presented data clearly indicates the terrain following method has met expectations, and allowed us to collect radiation data in quite constant distance from the ground regardless of the surface shape.

